A Language for the Declarative Composition of Concurrent Protocols

A recent study of bugs in real-world concurrent and distributed systems found that, while implementations of individual protocols tend to be robust, the composition of multiple protocols and its interplay with internal computation is the culprit for most errors. Multiparty Session Types and Choreographic Programming are methodologies for developing correct-by-construction concurrent and distributed software, based on global descriptions of communication flows. However, protocol composition is either limited or left unchecked. Inspired by these two methodologies, in this work we present a new language model for the safe composition of protocols, called Procedural Choreographies (PC). Protocols in PC are procedures, parameterised on the processes that enact them. Procedures define communications declaratively using global descriptions, and programs are written by invoking and composing these procedures. An implementation in terms of a process model is then mechanically synthesised, guaranteeing correctness and deadlock-freedom. We study PC in the settings of synchronous and asynchronous communications, and illustrate its expressivity with some representative examples.

==> conclusions.tex <==
We rock.

\fabrizio{The type system for graphs could be used in the future to check about fixed network structures, e.g., 
hypercubes.}
\fabrizio{Extensions are needed to reason about networks which do not follow divide-and-conquer.}

==> extend.tex <==
We now briefly discuss the characteristics we want to add to our minimal choreography
language AC, as well as how their inclusion changes this calculus.
%% In this section we briefly examine these five extensions separately, giving an intuition
%% of how AC needs to be changed to accommodate for them, and in some cases showing they do
%% not add any expressivity to AC on their own (although their combination with other
%% features does).
In the next section we introduce \ACrich, a choreography language incorporating all of
these primitives.

\subsection{Parameterized recursion}

Recursive procedures in AC are not allowed to take parameters.
However, this capability is needed in order to instantiate them with dynamically created
processes.
In the most general formulation, process variables $X$ take two sets of parameters,
$X(\pids q,\til x)$, and their calls instantiate them with process names and expressions,
$X\langle\pids p,\til e\rangle$.
However, in the minimalist setting of AC -- where processes only store one value -- the
second set is not necessary, as expressions can simply be stored in a particular process.

Extending AC by parameterizing process variables with a set of process names is
straightforward; furthermore, since AC does not feature the ability to spawn new
processes, this addition does not augment its expressive power.
Intuitively, since there is a finite number of process names, we can simply instantiate
all necessary values of the parameters in recursive definitions.

More concretely, writing \ACpar\ for the enriched calculus, we can define a mapping
$\unfold:\mbox{\ACpar}\to\mbox{AC}$ by
\begin{align*}
\unfold(\rec{X(\til q)}{A_2}{A_1}) ={} &\rec{X_1}{\unfold(A_2[\pids{p_1}/\pids q])}{}\\
  & \rec{X_2}{\unfold(A_2[\pids{p_2}/\pids q])}{}\\
  & \vdots \\
  & \rec{X_n}{\unfold(A_2[\pids{p_n}/\pids q])}{\unfold(A_1[X_i/X\langle\pids{p_i}\rangle])}
\end{align*}
where $X\langle\pids{p_1}\rangle,\ldots,X\langle\pids{p_n}\rangle$ are the recursive calls
to $X$ occurring in $A_1$, and $\unfold$ preserves all the remaining structure of an
\ACpar\ process.
Although there are exponentially many recursive calls in the expression above, this
recursion is terminating, as all of them are on structurally smaller processes.

\begin{theorem}
  \label{thm:recvars-bis}
  The relation $\{\langle A,\unfold(A)\rangle\mid A\in\mbox{\ACpar}\}$ is a bisimulation.
\end{theorem}

The definition of \unfold\ shows that the possibility of writing parameterized recursive
definitions can yield an exponential compression in the size of the choreographies.
It should be clear that this expansion is no longer possible in a calculus able to create
processes dynamically.

\subsection{Generalized sequential composition}
\label{sec:genseq}

In order to obtain general recursion rather than only tail recursion, we need to be able
to compose processes sequentially.
For technical reasons related to scoping, which impact the definition of EPP, it turns out
not to be convenient to define sequential composition in the most general way (i.e., to
add a rule $A;A$ to the grammar in Figure~\ref{fig:ac_syntax}), but rather to allow
choreographies of the form $(\gencond);A$, $(\genrec);A$ and $X;A$, as well as
$\nil;A$, which is needed as a runtime term.

We can then define an auxiliary general sequential composition $\fatsemi$ recursively as
follows.
\begin{align}
\label{eq:fatsemi}
(A_1;A_2)\fatsemi A_3 &= A_1;(A_2\fatsemi A_3)
& A\fatsemi A_3 &= A;A_3 & \mbox{ if $A$ is not of the form $A_1;A_2$}
\end{align}
This operator will be needed for the formal definition of the semantics of recursive
definitions; however, having it as a defined operation significantly simplifies the study
of the calculus.

The real gain in expressivity comes from the possibility of writing $X;A$: choreographies
not containing this construct can be translated to AC by replacing $A_1;A_2$ with
$A_1[A_2/\nil]$ whenever $A_1;A_2$ is not valid AC
syntax.\footnote{LCF: added next sentence. I don't think this is reasonable to include. :-)}
A formal proof of this result is beyond the scope of this paper.
However, this again gives a potentially exponential increase on the size of the
choreography, so again we gain in conciseness.

%% \begin{theorem}
%%   \label{thm:fatsemi-bis}
%%   The relation
%%   $\Delta_{\mbox{AC}}\cup\{\langle A_1\fatsemi A_2,A_1[A_2/\nil]\rangle\mid A_1,A_2\in\mbox{AC}\}$,
%%   where $\Delta_{\mbox{AC}}$ is the identity relation on AC choreographies, is a
%%   bisimulation up to $\preceq$.
%% \end{theorem}

%% An analysis of the proof of this theorem shows why the translation fails for $X;A$: even
%% though $X;A$ is trivially behaviourally equivalent to $X[A/\nil]$ (both have no
%% transitions), the fact that $\genrec;A'$ is behaviourally equivalent to $\genrec[A'/\nil]$
%% does not follow from the induction hypothesis and needs to be analysed
%% separately.\footnote{LCF: this theorem and its proof still need to be updated.}

\subsection{Type-aware processes}

Before we discuss spawning of new processes, it is convenient to address the issue of
including arbitrary datatypes in our calculus.
The original presentation of AC~\cite{ourstuff} focused on including a minimal set of
primitives to show Turing-completeness, and as such all process cells were uniformly typed
-- they stored natural numbers, which were the only available datatype, and could only
replace their contents by the input from a communication action.

In order to model a more realistic scenario, we need to consider different datatypes.
This can be done as follows:
\begin{itemize}
\item we assume a fixed set $\types$ of datatypes (numbers, lists, \ldots);
\item each process $\pid p$ can only store values of a fixed type $T_{\pid p}\in\types$;
\item communication actions have the form $\com{\pid p.e}{\pid q.f}$, where $f$ is a
  function of the form $\lambda x^T.t(\pcont)$, with intended semantics that $\pid q$
  combines the value received from $\pid p$ with its memory contents, as specified by
  function $f$, and stores the result.
\end{itemize}

The semantics of communication actions now also needs to check that the expression sent by
$\pid p$ has the type expected as input to $f$.
Furthermore, choreographies are now able to deadlock, as a process might try to send a
value of an incompatible type.
In order to deal with these problems, the resulting calculus will also need a (simple)
typing discipline to ensure that the usual good properties of choreographies are still
valid.
We will introduce this feature in Section~\ref{sec:types}.

AC trivially corresponds to restricting the set of types to $\types=\{\tnat\}$ and
replacing every communication $\gencom$ with $\com{\pid p.e}{\pid q.\m{id}}$.
It is straightforward to see that the (informally defined) restrictions on communication
actions are automatically satisfied.

The choice of functions allowed at the receiving end of communication actions, as well as
for building expressions, depends on the expressive power we want for our model.
If we want to model more realistic scenarios, as in Example~\ref{ex:mergesort}, we will
endow each process with powerful computational features and restrict communication between
processes.
If we want to minimize local computation and study the computational power of
communication alone, then we want to restrict our datatypes to minimal computation
features, corresponding to the usual constructors and destructors.
For example, we could restrict the functions on lists by allowing only sending of a list's
\verb+head+ or \verb+tail+, or the constant \verb+nil+, and receiving an element to be
\verb+cons+'ed to a process's list; in this case, we would need to implement a lower-level
variant of merge sort, where e.g.~the splitting step (the communication actions
\verb+q.split1 -> q1+ and \verb+q.split2 -> q2+) could be implemented as follows.

\begin{lstlisting}
def break(p,h):
	p start r in 
        	p.head -> h.cons; p.tail -> r.id; r.c -> p.id;

in def split(p,q1,q2):
	p.nil -> q1.id; p.nil -> q2.id;
        def X(q'1,q'2):
        	if p.isnil then 0
                else break(p,q'1); X<q'2,q'1>;
	in X<q1,q2>;

in split(q,q1,q2);
\end{lstlisting}

With this approach, types and process cells behave somewhat as classes and objects in
object-oriented programming: in a communication, the sender invokes one of its ``methods''
and sends the result; the receiver uses it as argument to one of its ``void methods''.

\subsection{Spawning new processes}

We now introduce the other important new ingredient absent from AC: the ability to start
new processes dynamically.
For this, we add a new unary start primitive $\genstart;A$, with intended semantics that
$\pid p$ creates a new process, hereby identified as $\pid q$ (but which will receive a
fresh name on execution), and whose type is $T$.
The expression $\genstart;A$ binds $\pid q$ in $A$.

At runtime, $\pid p$ is the only process who knows $\pid q$'s name.
In order for the EPP to work, we also need to extend the communication actions with the
ability to pass this information to other processes; also, the semantics for this extended
calculus needs to keep track of who knows who, and this condition must be verified in all
communication rules.
We therefore extend the semantics with a connection graph $G$, whose nodes are processes,
and whose edges correspond to the allowed communications.
We also introduce a new communication action $\gentell$, read ``$\pid p$ introduces
$\pid q$ and $\pid r$'', which adds an edge between $\pid q$ and $\pid r$ to $G$.
As its syntax suggests, this action consists of \emph{two} communication steps -- one where
$\pid p$ communicates $\pid q$'s name to $\pid r$, and another where $\pid p$ communicates
$\pid r$'s name to $\pid q$.
%% This makes total sense from an applicational point of view, as any process can only
%% communicate with processes it has previously been made aware of.

\subsection{Revised conditionals}

We end this section with a short note on conditionals.
In~\cite{ourstuff} we showed that a distributed conditional is necessary for
Turing completeness of AC, as the limited set of values one process can store is not
enough to perform comparisons.
However, when we allow richer types for process cells, we can restrict the conditional to
the result of a local computation: the conditional $\gencond$ from AC can be mimicked by
having $\pid p$ and $\pid q$ send their values to an auxiliary process with type
\m{nat\times nat}, which can then compare them locally.
In settings where processes store structured data (as the example at the beginning of this
section) this conditional is however a much more natural primitive to have.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> figures/apc_red_precongr.tex <==
\begin{figure}[t]
\footnotesize
\begin{eqnarray*}
&
\infer[\rname{C}{Com-Unfold}]
{
  \gencomf\ \precongrd\ \genasend;\asrecv{\pid p}{\pid q}fx
}
{}
\qquad
\infer[\rname{C}{Tell-Unfold}]
{
  \gentell\ \precongrd\ \genatell;\acom{\bullet_{\pid p}.\pid r}{\pid q}{x};\acom{\bullet_{\pid p}.\pid q}{\pid r}{y}
}
{}
\end{eqnarray*}
\caption{Asynchronous PC, Structural Precongruence (New Additional Rules).}
\label{fig:apc_red_precongr}
\end{figure}


==> figures/thetable.tex <==
% \newcommand{\yes}{yes}
% \newcommand{\no}{\text{\sffamily x}}
% \renewcommand{\partial}{\textasciitilde}
\begin{table*}
\centering
\begin{tabular}{c|ccccc}
  \multirow2*{Language} & Parameterised & General & Process & Transparent & Implicit \\
  & recursion & sequencing & spawning & EPP & parallelism \\ \hline
  MC~\cite{ourstuff} & no & no & no & yes & yes \\
  IOC~\cite{LGMZ08} & no & yes & no & yes & no \\
  DIOC~\cite{PGGLM15} & no & yes & no & no & no \\
  GC~\cite{CHY12} & no & no & partial & partial & no \\
  CC/Chor~\cite{CM13,M13:phd} & no & no & yes & yes & yes \\
  PC (this work) & yes & yes & yes & yes & yes \\
  \hline
\end{tabular}
% Notes for later.
% GC has process spawning but not explicit process variables, making parameterisation of procedures impossible.
% DIOC can spawn processes but not an unbounded number of them, maybe just say no and discuss.
% All these models ensure deadlock-freedom.
% Legend: \yes = yes, \no = no, \partial = partial
\caption{Expressive capabilities of representative choreography languages.}
\label{table:comparison}
\end{table*}
%


==> hopc.tex <==
\begin{figure*}
\footnotesize
\begin{eqnarray*}
&\infer[\rname{T}{EndSeq}]
{
  \Gamma;G\seq\nil;C \cseq G'
}
{
  \Gamma;G\seq C \cseq G'
}
\qquad
\infer[\rname{T}{Start}]{
  \Gamma;G\seq\genstart;C \cseq G'
}{
  \Gamma,\pid q:T;{\update{\pid p}{\pid q}} \seq C \cseq G'
}
\qquad
\infer[\rname{T}{Tell}]{
  \Gamma;G\vdash\gentell;C \cseq G'
}{
  \knows{\pid p}{\pid q} &
  \knows{\pid p}{\pid r} &
  \Gamma;\update{\pid q}{\pid r} \vdash C \cseq G'
}
\\[1ex]
&\infer[\rname{T}{Call}]
{
  \Gamma;G \seq \gencallP;C \cseq G'
}
{
	\Gamma \seq X(\wtil{\pid q^T}): G_X \cseq G'_X &
	% \Gamma_X[\pids p/\pids q] \subseteq \Gamma &
	\Gamma \seq \pid p_i:T_i &
	G_X[\pids p / \pids q] \subseteq G &
  \Gamma;G \cup (G'_X[\pids p/\pids q]) \seq C\cseq G'
}
\end{eqnarray*}
\caption{HO Procedural Choreographies, Typing Rules.}
\label{fig:pc_types}
\end{figure*}
%

